Illuminating the dark universe in the multi-messenger era

The precision era of multi-messenger astronomy, together with modern astrophysical, cosmological, and gravitational wave observations, increasingly points toward the existence of a ``dark" sector that cannot be explained within the framework of the Standard Model of particle physics and General Relativity. In this review, we explore extensions of standard physics and examine how observational data can be used to probe new particles and interactions. We consider a wide range of scales, from Solar System tests to galactic and cosmological observations, and investigate both conventional dark matter candidates, such as weakly interacting massive particles, and alternative scenarios including ultralight fields and primordial black holes. We discuss constraints derived from compact objects such as neutron stars, black holes, pulsars, and magnetars observations as well as from high-energy astrophysical phenomena. In addition, we analyze extensions of General Relativity involving additional scalar fields and their impact on gravitational wave signals and stochastic backgrounds from primordial black holes. We also study the capture and accumulation of dark matter in compact objects, which can alter properties such as mass, radius, and tidal deformability, and consider scenarios in which dark matter decays into Standard Model particles. While current observations already place significant limits on dark matter and modified-gravity models, upcoming experiments and observatories are expected to further probe or discover such new physics by improving constraints on particle masses and interaction strengths.

==> reviewanne/table_coefficients.tex <==
\begin{table}
\centering
\def\arraystretch{1.4}
\begin{tabular}{| @{\hspace{10pt}} l @{\hspace{15pt}} l @{\hspace{10pt}} |}
\hline
% ------ DIPOLE-DRIVE REGIME ------ %

% ------ QUADRUPOLE-DRIVE REGIME ------ %
\multicolumn{2}{|c|}{\small Quadrupole-driven regime}\\[2pt]
\hline
% Conformal [SO] nondip
$\begin{aligned}
\tablestyle
	\mathcal{S}_{\QD,\nondip}^\sector{C}
\\[5pt]~
\end{aligned}$
&
$\begin{aligned}
\tablestyle
	&
	\frac{1+2\alpha_1\alpha_2}{32\zeta\nu}
	\frac{5}{6}
	\bigg\{
		\frac{ \projell{S} }{\Geff m^2}
		\bigg(
			\frac{55-2\alpha_1\alpha_2}
				{1+2\alpha_1\alpha_2}
			-
			\frac{8}{\zeta}
		\bigg)
		\nonumber\\[-10pt]&
		-
		\frac{\projell\Sigma}{\Geff m^2}
		\bigg[
			\frac{ 5\comboA{+}{0}\comboA{\text{NLO}}{1} }
				{8\zeta\nu}
			-
			\bigg(
				\frac{27-2\alpha_1\alpha_2}
					{1+2\alpha_1\alpha_2}
				-
				\frac{33}{4\zeta}
			\bigg)
			\frac{\Delta m}{m}
		\bigg]
	\bigg\}
\end{aligned}$
\\[35pt]
% Conformal [SO] dip
$\begin{aligned}
\tablestyle
	\mathcal{S}_{\QD,\dip}^\sector{C}
\\[5pt]~
\end{aligned}$
&
$\begin{aligned}
\tablestyle
	&
	\frac{1+2\alpha_1\alpha_2}{32\zeta\nu}
	\frac{25\Delta\alpha^2}{336\zeta}
	\frac{7}{6}
	\bigg\{
		{-}
		\frac{ \projell{S} }{\Geff m^2}
		\bigg(
			\frac{65+2\alpha_1\alpha_2}{1+2\alpha_1\alpha_2}
			-
			\frac{48}{3\zeta}
		\bigg)
		\nonumber\\[-10pt]&
		-
		\frac{\projell{\Sigma}}{\Geff m^2}
		\bigg[
			\frac{ 6\comboA{+}{0} }{\Delta\alpha}
			-
			\frac{ 5\comboA{+}{0}\comboA{\text{NLO}}{1} }
				{4\zeta\nu}
			+
			\bigg(
				\frac{33 + 2\alpha_1\alpha_2}{1+2\alpha_1\alpha_2}
				-
				\frac{33}{2\zeta}
			\bigg)
			\frac{\Delta m}{m}
			\bigg)
		\bigg]
	\bigg\}
\end{aligned}$
\\[33pt]
% Disformal [SO] nondip
$\begin{aligned}
\tablestyle
	\mathcal{S}_{\QD,\nondip}^\sector{D}
\\[5pt]~
\end{aligned}$
&
$\begin{aligned}
\tablestyle
	&
	\frac{m}{2\pi\M^4(\Geff m)^3}
	\frac{1+2\alpha_1\alpha_2}{32\zeta\nu}
	\frac{5}{6}
	\sum_{\sigma=\pm}
	\frac{ \projell{S}_\sigma }{\Geff m^2}
	\nonumber\\[-10pt]&
	\times\!
	\bigg(
		\!-
		\frac{ 5\comboA{\text{NLO}}{1}\comboBS{-\sigma}{0} }
			{16\zeta\nu^2}
		-
		\frac{2\comboA{+}{2}\comboBS{-\sigma}{1}}
			{\zeta\nu^2}
		+
		\frac{52( \alpha_2^2\tilde\beta_1^\vph{2}
			+ \sigma\alpha_1^2\tilde\beta_2^\vph{2} ) }%
			{ 1 + 2\alpha_1\alpha_2 }
	\bigg)
\end{aligned}$
\\[33pt]
% Disformal [SO] dip
$\begin{aligned}
\tablestyle
	\mathcal{S}_{\QD,\dip}^\sector{D}
\\[5pt]~
\end{aligned}$
&
$\begin{aligned}
\tablestyle
	&
	\frac{m}{2\pi\M^4(\Geff m)^3}
	\frac{1+2\alpha_1\alpha_2}{32\zeta\nu}
	\frac{25\Delta\alpha^2}{336\zeta}
	\frac{7}{6}
	\sum_{\sigma=\pm}
	\frac{ \projell{S}_\sigma }{\Geff m^2}
	\nonumber\\[-10pt]&
	\times\!
	\bigg(
		\!-
		\frac{3\comboBS{-\sigma\,}{0}}{\Delta\alpha\nu}
		+
		\frac{ 5\comboA{\text{NLO}}{1}\comboBS{-\sigma}{0} }
			{8\zeta\nu^2}
		+
		\frac{4\comboA{+}{2}\comboBS{-\sigma}{1}}
			{\zeta\nu^2}
		-
		\frac{56( \alpha_2^2\tilde\beta_1^\vph{2}
			+ \sigma\alpha_1^2\tilde\beta_2^\vph{2} ) }%
			{ 1 + 2\alpha_1\alpha_2 }
	\bigg)
\end{aligned}$
\\[37pt]
\hline
\end{tabular}
\caption{Explicit expressions for the spin-orbit coefficients that appear in our solutions to the orbital and gravitational-wave phase. All of the symbols used above are defined in table~\ref{table:definitions}.}
\label{table:coefficients}
\end{table}

==> reviewanne/table_feyn_1.tex <==
\begin{table}
\centering
\begin{tabular}{|@{\hspace{10pt}} l @{\hspace{25pt}} l @{\hspace{25pt}} l @{\hspace{10pt}}|}
\hline
Diagram & Interaction vertex & Scaling \\
\hline
% Conformal [O]
\includegraphics[valign=c]{fig_rules_1_1}
&
$\tablestyle
\frac{\alpha_\K m_\K}{2\mpl}
\int\dx t\: \varphi$
&
$\sqrt{L}$
\\
% Conformal [SO]
\includegraphics[valign=c]{fig_rules_1_2}
&
$\tablestyle
\frac{\alpha_\K}{2\mpl}
\int\dx t\:
(S_\K^{i0} - S_\K^{ij}v_\K^j)\,\partial_i\varphi $
&
$\sqrt{L}v^2\epsSpin$
\\
% Disformal [O]
\includegraphics[valign=c]{fig_rules_1_3}
&
$\tablestyle
\frac{\beta_\K m_\K}{\M^4} \int\dx t\:
\dot\varphi^2$
&
$\tablestyle
\epsLadder e^2$
\\
% Disformal [SO]
\includegraphics[valign=c]{fig_rules_1_4}
&
$\tablestyle
\frac{\beta_\K}{\M^4}
\int\dx t\: S^{ij}_\K
(\partial_i\dot\varphi)\,\partial_j\varphi $
&
$\epsLadder\epsSpin$
\\[25pt]
\hline
\end{tabular}
\caption{Feynman rules for the four main worldline vertices. The scalar field is evaluated along the worldline; i.e., ${\varphi \equiv \varphi(t,\bm x_\K)}$, and  $\dot\varphi \equiv v_\K^\mu\partial_\mu\varphi$ for a total time derivative. Each factor of~$\varphi$ is  a dashed line, while the worldline  is a solid line. Vertices without black dots are spin-independent, while those with a black dot are coupled to one power of spin. The right column lists the power-counting rules for each vertex scales assuming all factors of~$\varphi$ are taken to be short-distance modes. If $\varphi$  is  taken  a radiation mode, include an extra factor of $\sqrt{v}$.}
\label{table:feyn_1}
\end{table}
